Gradient Cuff: Detecting Jailbreak Attacks on Large Language Models by Exploring Refusal Loss Landscapes

Large Language Models (LLMs) are becoming a prominent generative AI tool, where the user enters a query and the LLM generates an answer. To reduce harm and misuse, efforts have been made to align these LLMs to human values using advanced training techniques such as Reinforcement Learning from Human Feedback (RLHF). However, recent studies have highlighted the vulnerability of LLMs to adversarial jailbreak attempts aiming at subverting the embedded safety guardrails. To address this challenge, this paper defines and investigates the Refusal Loss of LLMs and then proposes a method called Gradient Cuff to detect jailbreak attempts. Gradient Cuff exploits the unique properties observed in the refusal loss landscape, including functional values and its smoothness, to design an effective two-step detection strategy. Experimental results on two aligned LLMs (LLaMA-2-7B-Chat and Vicuna-7B-V1.5) and six types of jailbreak attacks (GCG, AutoDAN, PAIR, TAP, Base64, and LRL) show that Gradient Cuff can significantly improve the LLM's rejection capability for malicious jailbreak queries, while maintaining the model's performance for benign user queries by adjusting the detection threshold.

==> experiments/comparison_smoothllm.tex <==
\subsection{Query Budget Analysis}
\label{smoothllm_compare}
 
Recall that we have discussed the approximation error of the gradient estimation in Section~\ref{subsec:grad_est}. We conclude that we can decrease the approximation errors by choosing larger values for $N$ and $P$. 

However, in Section \ref{subsec:gradient_cuff}
we show that the total query time cost $C_\theta(N,P,x)=N \cdot (P+1) \cdot t_\theta(x)$ would also increase with $N$ and $P$. We did ablation studies on $N$ and $P$ in Appendix~\ref{subapp:query_times} and found that it will have a better performance-efficiency trade-off when keeping $N$ fixed while changing $P$. Therefore, in this section, we fix $N=10$ and vary $P$  from $1$ to $10$ to evaluate Gradient Cuff under varying query times $q = N \cdot (P+1)$. As SmoothLLM also needs to query $T_\theta$ multiple times, we compare it with ours given the same query budget $q$. 


The results in Figure~\ref{fig:ptimes} show that 
when increasing the query budget, both SmoothLLM and our method would get better defense capability. The benign refusal rate for SmoothLLM is almost zero regardless of the number of query times, while the benign refusal rate for Gradient Cuff can be controlled by adjusting $\sigma$. 

Though SmoothLLM can maintain a similar benign refusal rate to Gradient Cuff when the $\sigma$ value is set to $5\%$, in terms of malicious refusal rate, Gradient Cuff outruns SmoothLLM by a large margin when the query times exceed $20$. For example, when allowing querying $T_\theta$ 110 times, Gradient Cuff can achieve $1.16 \times$ the malicious refusal rate of SmoothLLM on LLaMA2-7B-Chat and $1.80 \times$ the refusal rate on Vicuna-7B-V1.5.

==> impact.tex <==
\section{Impact Statement}
\label{sec:impact}
With the proliferation of LLMs and their applications across domains, reducing the risks of jailbreaking is essential for the creation of adversarially aligned LLMs. Our estimated impact is as broad as the LLMs themselves since safety alignment is fundamental to the development and deployment of LLMs. We do not currently foresee any negative social impact from this work.

==> pesudo_code/test.tex <==
\begin{algorithm}[thb!]
   \caption{Adaptive GCG}
   \label{alg:adaptive_gcg}
\begin{algorithmic}
\item \textbf{Input:} Initial prompt $x_{1:n}$, modifiable subset $\mathcal{I}$, iterations $T$, loss $\mathcal{L}$, $k$, batch size $B$
\State Word Embedding Layer of the protected language model $e_\theta(\cdot)$, Word Embedding Dimension $d$, Random Gaussian Vector generator $R$, Gradient Cuff perturb number $P$.
\State $V=R(P,d)$ \# generate P vectors each drawn from $\mathcal{N}(\mathbf{0},\mathbf{I})$ with dimension $d$
\For{$ T=1: \text{N}$}
\For{$i \in \mathcal{I}$}
\State $E=[e(x_{1:n}),e(x_{1:n})\oplus V_1, e(x_{1:n})\oplus V_2 \ldots, e(x_{1:n})\oplus V_P]$
\State $\mathcal{X}_i := \mbox{Top-}k(-\nabla_{e_{x_i}} \mathcal{L}(E))$ \#Compute top-$k$ promising token substitutions 
\EndFor
\For{$b=1:B$}
\State $\tilde{x}_{1:n}^{(b)} := x_{1:n}$ \#Initialize element of batch
\State $\tilde{x}^{(b)}_{i} := \mbox{UnIForm}(\mathcal{X}_i)$, where $i = \mbox{UnIForm}(\mathcal{I})$  \#Select random replacement token
\EndFor
\State $x_{1:n} = \tilde{x}^{(b^\star)}_{1:n}$, where $b^\star = \text{argmin}_{b} \mathcal{L}(\tilde{x}^{(b)}_{1:n})$ \#Compute best replacement
\EndFor
\end{algorithmic}
\end{algorithm}
